Federated Learning in ASR: Not as Easy as You Think

With the growing availability of smart devices and cloud services, personal speech assistance systems are increasingly used on a daily basis. Most devices redirect the voice recordings to a central server, which uses them for upgrading the recognizer model. This leads to major privacy concerns, since private data could be misused by the server or third parties. Federated learning is a decentralized optimization strategy that has been proposed to address such concerns. Utilizing this approach, private data is used for on-device training. Afterwards, updated model parameters are sent to the server to improve the global model, which is redistributed to the clients. In this work, we implement federated learning for speech recognition in a hybrid and an end-to-end model. We discuss the outcomes of these systems, which both show great similarities and only small improvements, pointing to a need for a deeper understanding of federated learning for speech recognition.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> parts/relate.tex <==
\section{Related work}\label{relatedwork}

Furthermore we take a look at federated averaging in general.

\subsection{Federated averaging}\label{sec:fedavg}
Federated averaging (\textit{FedAvg}) \cite{mcmahan2017communication} is commonly used as optimization method in a federated learning enviroment.
As shown in Algorithm~\ref{fadavg}, a pretrained model $\textit{\textbf{W}}^0$ initializes all clients at the beginning of the learning process.
Afterwards, the iterative optimization has two steps per round: 
%the local optimization, which is performed by each client and the global optimization step, which is executed by the server. In each of the traininig rounds, selected client models are initialized by the previous global model. Then the client models are updated with each clients private dataset. Finally, the \textit{FedAvg} is performed to update the global model.
the first step is the local optimization, which is performed by each client. The selected client models are initialized by the previous global model. To obtain the client local model, each client updated their model with their own dataset on-device. Then the FedAvg is applied over all selected client models. The averaged model is considered as the global model in this round and used in the next round.
In contrast to other works, which are averaging the accumulated gradient updates \cite{mcmahan2017communication, guliani2020training}, we averaged the model parameters (Equation~\ref{paramupdat}) at the end of each round.

\begin{algorithm}[htbp] 
\caption{Federated averaging. There are $N$ selected Clients are indexed by $n$, rounds are indexed by $i$. The pretrain dataset is $\textbf{D}_0$, The federated learning dataset for client n is denoted as $\textbf{D}_n$.}
\label{fadavg}
\begin{algorithmic}[1]
\STATE train the pretrained model with pretrain dataset $\textit{\textbf{W}}^0$ = \textit{Modeltraining}($\textbf{D}_0$).
\FOR{each round  $i = 1, 2, 3 \cdots$ }

\FOR{each client $n \in N$}
\STATE $\textit{\textbf{W}}^{i}_{n}$ = $\textit{\textbf{W}}^{i-1}$
\STATE $\textit{\textbf{W}}^{i}_{n}$ = \textit{Modeltraining}($\textbf{D}_n$)
\ENDFOR
\STATE $\textit{\textbf{W}}^{i} =\sum_{n}^{}\alpha_n\cdot \textit{\textbf{W}}^{i}_{n}, where \sum_{n}^{}\alpha_n = 1$
\ENDFOR

\end{algorithmic}
\end{algorithm}


\begin{equation}  \label{paramupdat}
\begin{aligned}
\textit{\textbf{W}}^{i} &=\sum_{n}^{}\alpha_n\cdot \textit{\textbf{W}}^{i}_{n}\\ 
&=\alpha_1\cdot (\textit{\textbf{W}}^{i-1} +\Delta \textit{\textbf{W}}^{i}_{1}) + \cdots 
 +\alpha_N\cdot (\textit{\textbf{W}}^{i-1} +\Delta \textit{\textbf{W}}^{i}_{N}) \\ 
&=\sum_{n}^{}\alpha_n\cdot \textit{\textbf{W}}^{i-1} + \sum_{n}^{}\alpha_n\cdot \Delta \textit{\textbf{W}}^{i}_{n} \\
&=\textit{\textbf{W}}^{i-1} + \sum_{n}^{}\alpha_n\cdot \Delta \textit{\textbf{W}}^{i}_{n}
\end{aligned}
\end{equation}

In Algorithm~\ref{fadavg}, the federated learning round could be performed with different communication frequencies. We can identify several communication frequency levels:
\begin{itemize}
\item $K$-Iterations level update (I-level): the communication is performed after every $K$ batches or chunks of training data or once the epoch is finished.
The selected client in every communication round checks, whether there are any untrained utterances for this client.
The client is removed if there is no more data to train in the current epoch.
This leads to a decline in the number of participants per round within the epoch.
After completion of an epoch of every speaker, a new round begins with the whole set of speakers participating again.

\item Epoch level update (E-level): update with the selected clients' models in every epoch. We can select all clients' models for the \textit{FedAvg} update, or alternatively, we can randomly select $N$ clients' models for updating.
\item Converge level update (C-level): update with the selected client models, these models are trained until convergent. So the model is only updated once with \textit{FedAvg}.
\end{itemize}
For \textit{FedAvg}, the averaging weights $\alpha_n$ in Algorithm~\ref{fadavg} could be defined as:
\begin{itemize}
\item  Mean average (M-average): $\alpha_n = \frac{1}{N}$, where $N$ is the number of the selected clients.
\item Weighted average (W-average): $\alpha_n = \frac{|\textbf{D}_n|}{\sum_{i}^{}|\textbf{D}_i|}$, where $|\textbf{D}_n|$ is the number of utterances of the federated learning dataset for the $n^\text{th}$ client .

\end{itemize}
%And the selected clients could be varied from randomly selected $N$ clients to contain all clients. 

